FuSeConv: Fully Separable Convolutions for Fast Inference on Systolic Arrays

Both efficient neural networks and hardware accelerators are being explored to speed up DNN inference on edge devices. For example, MobileNet uses depthwise separable convolution to achieve much lower latency, while systolic arrays provide much higher performance per watt. Interestingly however, the combination of these two ideas is inefficient: The computational patterns of depth-wise separable convolution are not systolic and lack data reuse to saturate the systolic array's constrained dataflow. In this paper, we propose FuSeConv (Fully-Separable Convolution) as a drop-in replacement for depth-wise separable convolution. FuSeConv generalizes the decomposition of convolutions fully to separable 1D convolutions along spatial and depth dimensions. The resultant computation is systolic and efficiently utilizes the systolic array with a slightly modified dataflow. With FuSeConv, we achieve a significant speed-up of 3x-7x with the MobileNet family of networks on a systolic array of size 64x64, with comparable accuracy on the ImageNet dataset. The high speed-up motivates exploration of hardware-aware Neural Operator Search (NOS) in complement to ongoing efforts on Neural Architecture Search (NAS).

==> content/related.tex <==
\noindent 

Several prior efforts have proposed alternate solutions for efficient DNN operators. The different efforts can be broadly grouped into the following categories. 

\textbf{Factorized Convolutions.} 
SqueezeNext \cite{gholami2018squeezenext} augmented the popular squeezeNet architecture and proposed the use of a two-stage squeeze module. One of the stages is composed of separable convolutions where the 3x3 spatial convolution in squeezeNet is replaced with two sequential blocks of 1x3 followed by 3x1 spatial convolution filters, while the other stage consists of element-wise addition. 
The use of separable convolutions reduced the total number of parameters and offered them significant benefits compared to squeezeNet. 
It is noteworthy, however, that the separable filters are spatial convolutions and are done sequentially. 
In contrast, we propose a fully-decomposed 1D convolution operation, across both the spatial and the depth axes, and the FuSe filters operate on the same input feature-map, offering us further benefits.  


\textbf{Improving Depthwise separable convolutions.} 
The problem of long runtimes for depthwise separable convolutions have been identified before and different solutions have been proposed to alleviate it.  



